GENEVA: Benchmarking Generalizability for Event Argument Extraction with Hundreds of Event Types and Argument Roles

Recent works in Event Argument Extraction (EAE) have focused on improving model generalizability to cater to new events and domains. However, standard benchmarking datasets like ACE and ERE cover less than 40 event types and 25 entity-centric argument roles. Limited diversity and coverage hinder these datasets from adequately evaluating the generalizability of EAE models. In this paper, we first contribute by creating a large and diverse EAE ontology. This ontology is created by transforming FrameNet, a comprehensive semantic role labeling (SRL) dataset for EAE, by exploiting the similarity between these two tasks. Then, exhaustive human expert annotations are collected to build the ontology, concluding with 115 events and 220 argument roles, with a significant portion of roles not being entities. We utilize this ontology to further introduce GENEVA, a diverse generalizability benchmarking dataset comprising four test suites, aimed at evaluating models' ability to handle limited data and unseen event type generalization. We benchmark six EAE models from various families. The results show that owing to non-entity argument roles, even the best-performing model can only achieve 39% F1 score, indicating how GENEVA provides new challenges for generalization in EAE. Overall, our large and diverse EAE ontology can aid in creating more comprehensive future resources, while GENEVA is a challenging benchmarking dataset encouraging further research for improving generalizability in EAE. The code and data can be found at https://github.com/PlusLabNLP/GENEVA.

==> abstract.tex <==
% Event Argument Extraction (EAE) is the task of extracting event-specific arguments from natural language sentences.
% Event Argument Extraction (EAE) models usually require a large amount of annotated data for training, but procuring annotations is expensive for each new event type.
To realistically cater to the emerging event types and new domains, it is essential for EAE models to be generalizable.
However, most standard EAE datasets like ACE and ERE have limited event diversity covering less than $40$ event types and $25$ argument roles,
which hinders them from adequately evaluating the generalizability of EAE models.
%To alleviate this issue, we make a three-fold contribution in our work. 
In this paper, we contribute a new dataset, \dataName{}, spanning the most diverse range of $115$ event types and $220$ argument roles to benchmark EAE models' generalizability.
% \tp{How to mention most diverse dataset in the above line?}
To build this dataset, we first create a large and diverse EAE ontology by transforming an existing semantic role labeling (SRL) dataset FrameNet.
% for the task of EAE 
For the same, we design ontology transfer mappings through exhaustive human expert annotations.
We then utilize these ontology mappings to create \dataName{} and conduct several human validation checks to ensure the high quality of our dataset.
% First, we study the relation between the tasks of semantic role labeling (SRL) and EAE, and devise a transfer mapping via exhaustive and extensive human expert annotations.
% Utilizing this transfer mapping, we construct \textit{a large EAE ontology} spanning a wide range of diverse event types and argument roles.
% To alleviate this issue, we utilize the relation between semantic role labeling (SRL) and EAE to first construct a large and diverse EAE ontology spanning 179 event types and 362 argument roles.
% Using this ontology, we create \dataName, a new EAE dataset covering a diverse range of 115 event types and 187 argument role types.
% Second, we create %a new large-scale EAE dataset 
% \dataName{} by repurposing an SRL dataset FrameNet based on our new ontology %spanning a diverse range of 115 event types and 220 argument roles 
% and conduct several human validation checks to ensure high quality for our dataset.
Using \dataName, we design four benchmarking test suites to evaluate generalizability of six EAE models
% from different model families 
in handling limited data and unseen event types.
% We design four benchmarking test suites using \dataName{} to assess the generalizability of EAE models in handling limited data and unseen event types. 
% Additionally, we propose a new model \modelName{} which establishes a strong benchmark on these test suites. 
% Third, we benchmark and evaluate the generalizability of recent EAE models from different model families
% and analyze their behaviors
% on the benchmarking test suites of \dataName.
% Our experiments reveal that DEGREE outperforms all other models and shows superior generalizability 
% \tp{Should we add line about DEGREE being best model in abstract?}.
Our experiments reveal how using generative-based models can yield superior generalizability and a performance boost of upto $30$ F1 points over traditional classification-based models.
% Our experiments reveal how utilizing pre-training language modeling objectives via label semantics and generation boosts generalization.
% Overall, we create a new most diverse EAE dataset \dataName{} and utilize it to benchmark the generalizability of EAE models.
\np{The final line/result is not compelling enough.}
\footnote{We will release our dataset and code upon acceptance.} 
% \ih{Remove numbers for contributions and reduce details or make it succinct. Make it more like a story. Write the contribution first and then mention details.}
% \violet{would be the best to also add some take-home messages on what're the shared challenges for all models.}
% Our experiments demonstrate the superior generalizability of %DEGREE and in general, 
% generation-based EAE models.
% \np{It looks like we did XYZ. Be more specific about the goals and contributions. the last sentence needs to be strong take-home message.}
% \kw{Write more about our contributions. Remove the initial motivation.}

% % Numerous events occur worldwide and are documented in news, social media, and various online platforms in raw text.
% % Extracting useful and succinct information about these events is crucial to various downstream applications.
% Event Argument Extraction (EAE) deals with the task of extracting event-specific information from natural language text.
% EAE models usually require annotated data for training, but procuring annotations is expensive for each new event type.
% % \kh{Add line about no/few training data}
% % \ih{Hard to collect annotations and data is low realistically.}
% To cater to the emerging event types and new domains in a realistic setting, %there is a growing urgency 
% it is growingly imperative 
% for EAE models to be generalizable.
% %Consequentially, there is a necessity for benchmarking setups to evaluate the generalizability of EAE models.
% % \ih{Move this above and motivate for new events after this line}
% However, most existing benchmark datasets like ACE and ERE have limited coverage in terms of event types and cannot adequately evaluate the generalizability of EAE models.
% % Most existing works benchmark their model performance on the standard datasets of ACE and ERE.
% % But these datasets have limited coverage in terms of the unique number of events and argument roles and thus, they cannot adequately evaluate the models on a diverse set of events.
% % To alleviate this issue, we introduce a new Generalizability bENchmarking dataset for EVent Argument extraction (GENEVA) covering a diverse range of 115 events and 187 argument roles.
% To alleviate this issue, we introduce \dataName, a new dataset  covering a diverse range of 115 event types and 187 argument role types.
% We create four benchmarking test suites in \dataName{} to assess EAE models' generalizability.
% % We use our dataset to set up few-shot and zero-shot benchmarking test suites to test the generalizability of models.
% Additionally, we propose a new model \modelName{} which establishes a strong benchmark on these test suites.
% Lastly, we evaluate the generalizability of several recent EAE systems from different model families and analyze their behavior on \dataName.\footnote{We will release our dataset and code upon acceptance.}
% % along with our proposed model \modelName, focusing on the generalizability of EAE to establish strong baselines as well as highlighting the challenges of the proposed dataset. %on these test suites and compare their generalizability relatively.
% %Finally, we propose a new model GENEVA that outperforms the previous models and serves as a strong benchmark for these test suites.
% % We introduce a new model DAM with automated refinements on DEGREE.

==> abstract_text.tex <==
Recent works in Event Argument Extraction (EAE) have focused on improving model generalizability to cater to new events and domains. However, standard benchmarking datasets like ACE and ERE cover less than 40 event types and 25 entity-centric argument roles. Limited diversity and coverage hinder these datasets from adequately evaluating the generalizability of EAE models. In this paper, we first contribute by creating a large and diverse EAE ontology. This ontology is created by transforming FrameNet, a comprehensive semantic role labeling (SRL) dataset for EAE, by exploiting the similarity between these two tasks. Then, exhaustive human expert annotations are collected to build the ontology, concluding with 115 events and 220 argument roles, with a significant portion of roles not being entities. We utilize this ontology to further introduce GENEVA, a diverse generalizability benchmarking dataset comprising four test suites aimed at evaluating models' ability to handle limited data and unseen event type generalization. We benchmark six EAE models from various families. The results show that owing to non-entity argument roles, even the best-performing model can only achieve 39% F1 score, indicating how GENEVA provides new challenges for generalization in EAE. Overall, our large and diverse EAE ontology can aid in creating more comprehensive future resources, while GENEVA is a challenging benchmarking dataset encouraging further research for improving generalizability in EAE.

==> conclusion.tex <==
\section{Conclusion and Future Work}

\tp{To be updated}
In this paper, we introduce a new diverse EAE dataset \dataName{} comprising of a wide range of event types and argument roles.
% We demonstrate the distinctiveness and the realistic nature of our dataset compared to previous datasets via several data analyses.
We develop four benchmarking test suites for evaluating model generalizability on the dataset and 
% in limited and no training data settings to extensively evaluate the generalizability of EAE models.
benchmark various representative EAE models.
% and compare their generalizability.
We also propose \modelName{} which shows superior generalization across the different test suites.
% and serves as a strong baseline.
Future work includes expansion of this dataset to cover more diverse event types and argument roles.
Efforts can also be taken to improve the automated heuristics for \modelName{} and in turn, pushing the limit of generalizability furthermore.


==> data.tex <==
\section{\dataName{} Dataset}
\label{sec:geneva-dataset}

% \begin{table*}[t]
%     \centering
%     \small
%     \begin{tabular}{l|l|l|l}
%         \toprule
%         \textbf{Frame} & \multicolumn{1}{|c}{Arrest} & \multicolumn{1}{|c}{Visiting} & \multicolumn{1}{|c}{Travel} \\ \hline
%         & Authorities, Charges, Offense, & \textcolor{orange}{Agent,} \textcolor{blue}{Entity,} \colGray{\textit{Frequency},} & \textcolor{orange}{Traveler,} \textcolor{purple}{Path,} Source, \textcolor{blue}{Goal,} Direction, \\
%         & Suspect, \colGray{\textit{Co-participant},} \colGray{\textit{Time},} & \colGray{\textit{Depictive},} \colGray{\textit{Duration},} \colGray{\textit{Means},} & Mode of Transportation, \textcolor{purple}{Area,} \colGray{\textit{Explanation},} \\
%         \textbf{Frame} & \colGray{\textit{Means},} \colGray{\textit{Place},} \colGray{\textit{Purpose},} \colGray{\textit{Type},} & \colGray{\textit{Iterations},} \colGray{\textit{Manner},} \colGray{\textit{Purpose},} & \colGray{\textit{Frequency},} \colGray{\textit{Baggage},} \colGray{\textit{Depictive},} \colGray{\textit{Iterations},} \\
%         \textbf{Elements} & \colGray{\textit{Source of legal authority},} & \colGray{\textit{Normal location},} \colGray{\textit{Place},} & \colGray{\textit{Co-participant},} \colGray{\textit{Duration},} \colGray{\textit{Manner},} \colGray{\textit{Speed},} \\
%         & \colGray{\textit{Manner}} & \colGray{\textit{Dependent state},} \colGray{\textit{Time}} & \colGray{\textit{Time},} \colGray{\textit{Descriptor},} \colGray{\textit{Period of iterations},} \\
%         & & & \colGray{\textit{Distance},} \colGray{\textit{Means},} \colGray{\textit{Purpose},} \colGray{\textit{Result}} \\
%         % & \textcolor{green}{Authorities,} \textcolor{orange}{Charges,} \textcolor{yellow}{Offense,} & \textcolor{red}{Agent,} \textcolor{blue}{Entity,} \colGray{Frequency,} & \textcolor{red}{Traveler,} \textcolor{cyan}{Path,} \textcolor{magenta}{Source,} \textcolor{blue}{Goal,} \colGray{Explanation,} \\
%         % & \textcolor{pink}{Suspect,} \colGray{Co-participant,} \colGray{Time,} & \colGray{Depictive,} \colGray{Duration,} \colGray{Means,} & \textcolor{violet}{Mode of Transportation,} \textcolor{cyan}{Area,} \colGray{Frequency,} \\
%         % \textbf{Frame} & \colGray{Means,} \colGray{Place,} \colGray{Purpose,} \colGray{Type,} & \colGray{Iterations,} \colGray{Manner,} \colGray{Purpose,} & \textcolor{brown}{Direction,} \colGray{Baggage,} \colGray{Depictive,} \colGray{Iterations,} \\
%         % \textbf{Elements} & \colGray{Source of legal authority,} & \colGray{Normal location,} \colGray{Place} & \colGray{Co-participant,} \colGray{Duration,} \colGray{Manner,} \colGray{Speed,} \\
%         % & \colGray{Manner} & \colGray{Dependent state,} \colGray{Time} & \colGray{Time,} \colGray{Descriptor,} \colGray{Period of iterations,} \\
%         % & & & \colGray{Distance,} \colGray{Means,} \colGray{Purpose,} \colGray{Result} \\
%         % \textcolor{red}{Agent,} \textcolor{blue}{Entity,} \colGray{Dependent state,} \\
%         % & \colGray{Depictive,} \colGray{Duration,} \colGray{Frequency,} \\
%         % & \colGray{Iterations,} \colGray{Manner,} \colGray{Means,} \colGray{Time,} \\
%         % & \colGray{Normal location,} \colGray{Purpose,} \colGray{Place} \\
%         % & \textcolor{cyan}{Area,} \textcolor{cyan}{Path,} \textcolor{magenta}{Source,} \textcolor{blue}{Goal,} \\
%         % & \textcolor{violet}{Mode of Transportation,} \textcolor{red}{Traveler,} \\
%         % & \textcolor{brown}{Direction,} \colGray{Baggage,} \colGray{Depictive,} \\
%         % & \colGray{Descriptor,} \colGray{Distance,} \colGray{Means,} \\
%         % & \colGray{Duration,} \colGray{Manner,} \colGray{Frequency,} \colGray{Time,} \\
%         % & \colGray{Iterations,} \colGray{Period of iterations,} \\
%         % & \colGray{Purpose,} \colGray{Result,} \colGray{Travel Means,} \\
%         % & \colGray{Co-participant,} \colGray{Explanation,} \colGray{Speed} \\
%         \bottomrule
%     \end{tabular}
%     \caption{An illustration of the complex structure for different frames from FrameNet.
%     During \dataName creation, frame elements in the same color are merged into a single argument role, while those in \colGray{\textit{italics}} are filtered out.
%     \tp{Need to update example. Takes too much space and difficult to understand directly.}
%     }
%     \label{tab:framenet-example}
% \end{table*}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.98\textwidth]{images/geneva-creation.pdf}
%     \caption{Figure highlighting the various operations performed to create our proposed EAE dataset \dataName{} from the SRL dataset FrameNet.
%     \tp{Figure to be removed/updated.}}
%     \label{fig:data-creation}
%     \vspace{-1em}
% \end{figure*}

% Although the EAE ontology can be used in different ways,
Using our large and diverse EAE ontology, we now construct a new diverse EAE dataset \dataName{} for evaluating the generalizability of models.
Annotating data for EAE for such a wide set of events is a resource-heavy and expensive process.
Rather, we utilize the annotations from FrameNet dataset to build \dataName{}.
% We follow the event definition from ACE \cite{doddington-etal-2004-automatic} (described in Appendix~\ref{sec:task-def}).
We provide details about our data creation process in \S~\ref{sec:data-creation} and provide data statistics in \S~\ref{sec:data-analysis}.
% \tp{Some reference to image once its ready}
% and introduce generalizability benchmarking test suites in \S~\ref{sec:benchmark-setup}.

% \subsection{FrameNet for EAE}
% \label{sec:framenet-eae}

% SRL and EAE are similar tasks in that SRL assigns semantic roles to phrases in the sentence and EAE aims at extracting event-specific argument roles from the sentence.
% Owing to these similarities, we utilize FrameNet \cite{baker-etal-1998-berkeley-framenet}\footnote{FrameNet Data Release 1.7 by \url{http://framenet.icsi.berkeley.edu} is licensed under a Creative Commons Attribution 3.0 Unported License.} - a comprehensive SRL dataset comprising of 1200+ semantic frames \cite{fillmore1976frame} - to create an EAE dataset.
% % Owing to these similarities, we utilize FrameNet \cite{baker-etal-1998-berkeley-framenet} which is primarily a SRL dataset annotated by expert linguists \cite{gildea-jurafsky-2000-automatic}, to create an EAE dataset.
% % The annotation schema for FrameNet follows the theory of Frame Semantics \cite{fillmore1976frame, fillmore2010frames} and it comprises of 1200+ semantic frames.
% The definition of a \textit{frame} is rather loose and can be understood as the holistic background that unites similar words.\footnote{\url{www.web.stanford.edu/~jurafsky/slp3/19.pdf}}
% Each frame is annotated with frame-specific semantic roles (\textit{frame elements}) and words that evoke the frame (\textit{lexical units}).
% We utilize FrameNet for EAE by mapping selective \textit{frames} that have "Event" relations as events.
% Correspondingly, we can map the \textit{lexical units} as event triggers and \textit{frame elements} as argument roles.
% % We utilize FrameNet for EAE by mapping \textit{frames} as events, \textit{lexical units} as event triggers and \textit{frame elements} as argument roles \cite{wang-etal-2020-maven}.
% For example in Table~\ref{tab:framenet-example}, the frame \textit{Arrest} and its frame elements can be mapped to the event \textit{Arrest-Jail} of the ACE dataset and its argument roles respectively. 

% However, the applicability of FrameNet for EAE has been limited.
% % due to the inherent difference between the tasks of Semantic Role Labeling and Event Argument Extraction.
% This is primarily because FrameNet 
% % is an SRL dataset that 
% prioritizes lexicographic and linguistic completeness \cite{aguilar-etal-2014-comparison},
% % On the other hand,
% % \sdl{I don't quite get why we dropped "On the other hand" as the transition word here}
% while EAE is a higher-level task requiring extraction of distinct and succinct information.
% % \ih{Talk about how event extraction is different and need to extract clear and succinct information.}
% % \kw{Don't call it drawbacks. Talk about the difference between SRL and EAE. Then discuss the difficulties in transfer.}
% This difference leads to two major challenges in using FrameNet for EAE:
% (1) \textit{FrameNet frames are too fine-grained and many times indistinguishable from the aspect of EAE}, and 
% (2) \textit{FrameNet frames have a complex structure comprising of a wide range of frame elements which may all not be relevant for EAE}.
% % \sdl{probs need to restructure (1), I still feel kinda confused even after reading it; also you probs need to highlight them using textbf/textbb}
% % \ih{Add some conclusion. Broad idea of what you want to do.}
% % are complex objects containing a wide number of frame elements and intricate relations between them.
% % We also observe the complex and wide-range of frame elements, which can not be all used directly for EAE.
% % \tp{Adding more examples}

\begin{table*}[!ht]
    \centering
    \small
    \begin{tabular}{lrrrrrrr}
    \toprule
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\#Sentences}} & \textbf{\#Event} & \textbf{\#Arg} & \textbf{\#Event} & \textbf{\#Arg} & \textbf{Avg. Event} & \textbf{Avg. Arg} \\
        & & \textbf{Types} & \textbf{Types} &\textbf{Mentions} & \textbf{Mentions} & \textbf{Mentions} & \textbf{Mentions} \\
    \midrule
        ACE & 18,927 & 33 & 22 & 5,055 & 6,040 & 153.18 & 274.55 \\
        ERE & 17,108 & 38 & 21 & 7,287 & 10,479 & 191.76 & 499 \\
        \dataName & 3,673 & 115 & 220 & 7,505 & 12,269 & 65.26 & 55.77 \\
    \bottomrule
    \end{tabular}
    \caption{
    \looseness=-1
    Statistics for the different datasets for Event Argument Extraction. The third and fourth columns indicate the unique number of event types and argument roles. The fifth and sixth column are the number of event and argument mentions in the dataset. The last two columns indicate the average number of mentions per event and argument role.
    \np{Too much space but not too much info.}}
    \label{tab:dataset-coverage}
    \vspace{-3mm}
\end{table*}

\subsection{Creation of \dataName}
\label{sec:data-creation}

% FrameNet is primarily an SRL dataset and cannot be readily transferred for the task for EAE.
% Utilizing the EAE ontology created in Section~\ref{sec:event-arg-building}, we perform the following set of steps to transfer the FrameNet dataset into \dataName{} for EAE.

% We first transfer FrameNet dataset to create \dataName{} and conduct human validation to ensure high quality of the annotations.

% \mypar{FrameNet Transfer}
% In order to transfer FrameNet for EAE, we first map the dataset using the EAE ontology.
Along with frame schema, FrameNet also comprises dataset of annotated sentences.
% We utilize the EAE ontology to perform three mapping steps on the FrameNet dataset: (1) Mapping each frame to a corresponding event, (2) Mapping lexical units as event triggers, and (3) Mapping each frame element to a corresponding event argument role.
We utilize the previously designed ontology mappings to repurpose the annotated sentences from FrameNet for EAE by mapping frames to corresponding events, lexical units to event triggers, and frame elements to corresponding arguments.
Unmapped frames and frame elements (not present in the EAE ontology) are filtered out from the dataset.
Since FrameNet doesn't provide annotations for all frames, some events from the ontology have no data in our dataset.
To aid better evaluation, we
% further set a minimum data requirement for each event to 5 event mentions (in order to aid better evaluation) and 
remove events that do have less than $5$ event mentions (e.g. \textit{Lighting}).
% Lexical units in FrameNet sentences are mapped as event triggers for EAE.
% Finally, sentences with no event mentions are also removed from the dataset.
Our final dataset \dataName{} comprises  115 event types and 220 argument roles.
Some examples are provided in Figure~\ref{fig:dataset-examples} (Appendix).

\mypar{Human Validation:}
% \tp{Update after comprehensiveness test is done}
We ensure high quality of our dataset by conducting two human assessments:

\noindent (1) Ontology Quality Assessment:
% In order to distinguish \dataName{} from FrameNet and validate the utility of our merging operations, we set up a human validation experiment (Step 6).
We present the human annotators with three sentences - one primary and two candidates - and ask them if the event in the primary sentence is similar to the events in either of the candidates or distinct from both (Example in Appendix~\ref{sec:human-validation-setup}).
One candidate sentence is chosen from the frame merged with the primary according to our ontology, while the other candidate is chosen from a similar unmerged sister frame.
% , which is a sibling event of the primary event discovered from the event ontology.
% unmerged frame\footnote{Similarity measured by sister nodes in the event ontology.}.
% We present the human experts with a pair of event mentions of two frames that were merged for \dataName{} and ask if the event types in the sentences are similar.
% As a strong baseline, we also present them with a pair of event mentions from very similar unmerged frames.\footnote{Similarity measured by sister nodes in the event ontology.}
The annotators chose the merged frame candidates $87\%$ of the times.
This validation was done by three annotators over $61$ sampled triplets and with $0.7$ IAA measured by Fleiss' kappa \cite{fleiss1971measuring}.

\noindent (2) Annotation Comprehensiveness Assessment:
Human annotators are presented with annotated samples from our dataset and they are asked to report if there are any arguments in the sentence that have not been annotated.
The annotation is comprehensive if all arguments are annotated correctly.
The annotators reported that the dataset annotations were $89\%$ comprehensive.
Major corrections mainly comprised ambiguous cases and incorrect role assignments.
% \tp{add results and analysis}
This assessment was done by two expert annotators over $100$ samples from the dataset with a IAA of $0.93$ (Cohen's kappa).
% These human validations ensure the quality of our dataset.
% quality as well as underlines the significance of the various operations performed for the creation of \dataName.

\subsection{Data Analysis}
\label{sec:data-analysis}

% \tp{Update Statistics and this section}
The major statistics for \dataName{} are shown in Table~\ref{tab:dataset-coverage} along with its comparison with sentence-level EAE datasets ACE and ERE.
We discuss some charaterstics of our dataset below.
% Based on these statistics, we show how \dataName{} is more diverse, challenging, and dense in nature, and in turn,
% is distinct from previous EAE datasets of ACE and ERE, and
% better suited for evaluating the generalizability of EAE models.
% Towards this end, we provide various data analyses to support these claims.

\noindent \textbf{Diverse:}
\dataName{} has a wide coverage with thrice the number of event types and 10 times the number of argument roles relative to ACE/ERE.
% (third and fourth columns in Table~\ref{tab:dataset-coverage}).
We categorize the events in these datasets into abstract event types (as defined in MAVEN) and present their distributions in Figure~\ref{fig:ace-in-geneva}.
The figure depicts how ACE/ERE events are concentrated only in specific abstractions of Action and Change, while \dataName{} is the most diverse with events from $5$ abstract types.

\noindent \textbf{Challenging:}
% Furthermore, the number of event and argument role mentions are more compared to the previous datasets.
Due to higher number of event types and argument roles, the average number of mentions per event type and argument role (last two columns in Table~\ref{tab:dataset-coverage}) is much lesser for \dataName{}.
Consequently, this makes training models more challenging as models need to train from fewer examples on average.

% Overall, these statistics show how \dataName{} is more diverse and challenging than the previous datasets.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/ace-in-geneva-circular.pdf}
%     \caption{Distribution of event types by the number of event mentions in GENEVA.}
%     \label{fig:event-data-distribution}
% \end{figure}

% Due to the high number of unique events and arguments, \dataName is a dense dataset with an average of 2 events and 3 arguments per sentence (can be observed from Table~\ref{tab:dataset-coverage}).
% We further also plot the percentage distribution of event mentions per sentence for ACE, ERE, and FN-115 in Figure~\ref{fig:event-mention-density}\footnote{Since FN-115 doesn't have any sentence with zero event mentions, we remove sentences with zero event mentions in the distribution for ACE and ERE as well}.
% We can clearly observe that ACE and ERE have more than $65\%$ of the sentences with a single event mention, whereas FN-115 has $65\%$ with 2 or more event mentions.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/event-mention-density.png}
%     \caption{Event mention density as percentage of data for ACE, ERE and FN-115 datasets.}
%     \label{fig:event-mention-density}
% \end{figure}

\noindent \textbf{Dense:}
Although \dataName{} has fewer sentences compared to the other datasets, it has more number of event and argument role mentions (fifth and sixth columns in Table~\ref{tab:dataset-coverage}).
This makes \dataName{} a highly dense dataset in terms of mentions per sentence.
% with an average of 2 events and 3 arguments per sentence (can be deduced from Table~\ref{tab:dataset-coverage}).
We plot the distribution of arguments per sentence\footnote{We remove no event mention sentences for ACE/ERE.} for ACE, ERE, and \dataName{} in Figure~\ref{fig:argument-mention-density}.
% We observe that more than $25\%$ of the sentences have zero argument mentions for ACE.
Both ACE and ERE have a high proportion of sentences ($>70\%$) with up to 2 argument roles.
% \ih{Just mention the high density arguments and not mention that ACE/ERE have low}
% \ih{ACE, ERE are sparse because the base resource is a single , while GENEVA is sentence-picked. Add it as a footnote.}
% \sdl{same suggestion as previous ones, I would recommend us to check all usage of ``on the other hand'' through the draft to see if we have better transition words for each of those places}
In contrast, \dataName{} is denser with almost $50\%$ of sentences having 3 or more arguments and more than $20\%$ of sentences with 5+ arguments.
% \tp{Some conclusion to have here}
% \np{Dense dataset is a good dataset.}
% This dense nature of FN-115 makes the task of EAE relatively more difficult.
% We further also plot the percentage distribution of event mentions per sentence for ACE, ERE, and FN-115 in Figure~\ref{fig:event-mention-density}\footnote{Since FN-115 doesn't have any sentence with zero event mentions, we remove sentences with zero event mentions in the distribution for ACE and ERE as well}.
% We can clearly observe that ACE and ERE have more than $65\%$ of the sentences with a single event mention, whereas FN-115 has $65\%$ with 2 or more event mentions.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/argument-mention-density.pdf}
    \caption{Arguments per sentence as percentage of data for ACE, ERE and \dataName{} datasets.
    \np{Violin plots for three datasets.}
    % \sdl{it could be helpful if we introduce an envelope curve for each of the dataset so that the concept of being \emph{diverse} can be more clearly illustrated? Or use some meaure to quantify this. Otherwise I don't think we can safely claim that the distribution of GENEVA is statistically-significantly more diverse.}
    }
    \label{fig:argument-mention-density}
    \vspace{-3mm}
\end{figure}

Overall, \dataName{} is a dense, challenging and the most diverse EAE dataset.
These characterstics make \dataName{} better-suited than existing datasets for evaluating the generalizability of EAE models.


==> eae_task.tex <==
% \section{Event Argument Extraction Task}

% \tp{Formally introducing the task of event extraction and EAE}

% Event Extraction (\textbf{EE}) comprises of two subtasks - Event Detection (\textbf{ED}) and Event Argument Extraction (\textbf{EAE}).
% ED involves the task of identifying event triggers in a sentence and classifying them into event types.
% EAE utilizes the event triggers (as inputs) to identify event argument roles related to the event in the given sentence.
% We provide an example of the two tasks by an example as shown in Figure~\ref{fig:ee-example}.
% In our work, we focus our efforts on scaling up and improving the benchmarks for the task of EAE.

% Expanded version for WQE
% Event Extraction (\textbf{EE}) is a structured prediction task aimed at identifying events and extracting specific event-related information from natural language text.
% It comprises of two subtasks - Event Detection (\textbf{ED}) and Event Argument Extraction (\textbf{EAE}).
% ED involves the task of identifying words (also called event triggers) which indicate events in a sentence and classifying them into a pre-defined list of event types.
% EAE utilizes this event-type information (as inputs) to identify and classify event-specific roles (also called argument roles) in the given sentence.
% We provide an illustration of the two tasks by an example sentence in Figure~\ref{fig:ee_example}.
% In our work, we focus on improving the benchmarks for the task of EAE.

\section{Event Argument Extraction Definition}

\tp{Should it be a separate section?}

\np{Maybe blend it in the intro in the 1st para.}

We describe the task of Event Argument Extraction (EAE) formally along with its associated technical terminologies. 
An \textbf{event} is a specific occurrence involving multiple participants and is labeled with a specific \textbf{event type}. 
An \textbf{event mention} is a sentence in which the event is described. 
An \textbf{event trigger} is a word phrase which expresses the event occurence in an event mention. 
An \textbf{event argument} is a word phrase that mentions an event-specific attribute or participant and is labeled with a specific \textbf{argument role}.
EAE deals with the task of identifying event arguments in event mentions and classifying them into argument roles.
EAE models can utilize event type and the associated event trigger as additional information for the task.

==> experiments.tex <==
\section{Experimental Setup}

% In this section, we discuss the different benchmarking setup for our experiments, introduce the different baseline models, and finally describe the evaluation metrics.
We evaluate the generalizability of various EAE models by designing four benchmarking test suites using \dataName.
We describe these test suites in \S~\ref{sec:benchmark-setup}, the benchmarked EAE models in \S~\ref{sec:models} and the evaluation metrics in \S~\ref{sec:eval-metrics}.
% In this section, we describe our experimental setup comprising of the various EAE models (\S~\ref{sec:models}) and the evaluation metrics (\S~\ref{sec:eval-metrics}).

\subsection{Benchmarking Test Suites}
\label{sec:benchmark-setup}

With a focus on the evaluation of the generalizability of the EAE models, we fabricate four benchmarking test suites clubbed into two higher-level settings, as described below:

% \paragraph{Limited Training Data}
\mypar{Limited Training Data:}
This setting mimics the realistic scenario when there are fewer annotations available for the target events and evaluates models' ability to learn from limited training data.
We present two test suites for this setting: 
\begin{itemize}[topsep=1pt, itemsep=-3pt, leftmargin=13pt]
    \item Low resource (LR): Training data is created by \textit{randomly} sampling $n$ event mentions.
    \footnote{To discount the variance of number of event mentions per sentence, we create the sampled training data such that each of them has a fixed number of $n$ event mentions.}
    % \footnote{Due to a high variation in the number of event mentions per sentence, a fixed number of sampled sentences could have a varied number of event mentions. To discount this variability, we create the sampled training data such that each of them has a fixed number of $n$ event mentions.}
    We record the model performance across a spectrum from extremely low resource ($n=1$) to moderately resource ($n=1200$) settings.
    \item Few-shot (FS): Training data is curated by sampling $n$ event mentions \textit{uniformly} across all events. This sampling strategy avoids biases towards high data events and assesses the model's ability to perform well uniformly across events. We study the model performance from one-shot ($n=1$) to five-shot ($n=5$) for this test suite.
% We record the model performance across a spectrum from extremely low resource ($n=1$) to moderately resource ($n=1200$) settings.
\end{itemize}
% \textbf{(1) Low resource (LR)} and \textbf{(2) Few-shot (FS)}.
% For the low resource test suite, we create training data by randomly sampling $n$ event mentions.\footnote{Due to a high variation in the number of event mentions per sentence, a fixed number of sampled sentences from the training data could have a varied number of event mentions. To discount this variability, we create the sampled training data such that each of them has a fixed number of $n$ event mentions.}
% We record the model performance across a spectrum from extremely low resource ($n=1$) to moderately resource ($n=1200$) settings.
% For the few-shot test suite, we create training data by sampling $n$ event mentions \textit{uniformly} across all events.
% This sampling strategy avoids biases towards high data events and assesses the model's ability to perform well uniformly across events.
% We study the model performance from one-shot ($n=1$) to five-shot ($n=5$) for this test suite.
% % For both the test suites, we sample 5 different datasets\footnote{We release all these different datasets for reproducibility and future benchmarking.} for each setup and report the average model performance to account for the sampling variation.
% The test dataset is consistent across the two test suites and corresponding statistics is shown in Table~\ref{tab:data-split}.

% \paragraph{Unseen Event Data}
\mypar{Unseen Event Data:}
The second setting focuses on the scenario when there is no annotation available for the target events. This helps test models' ability to generalize to unseen events and argument roles.
We propose two test suites: %\textbf{(1) Zero-shot (ZS)} and \textbf{(2) Cross-type Transfer (CTT)}.

\begin{itemize}[topsep=1pt, itemsep=-3pt, leftmargin=13pt]
    \item Zero-shot (ZS): The training data comprises the top $m$ events with most data, where $m$ varies from 1 to 10. \footnote{We sample a fixed $450$ sentences for training to remove the variance of dataset size for different $m$.}
    The remaining 105 events are used for testing.
    % Intending to study the impact of event diversity on the zero-shot model performance, we create three training datasets by sampling a fixed 450 sentences\footnote{Fixing the training data size removes the confounding variable of data size for the study.} for $m$ events from the larger training corpus. We vary $m$ from 1 to 10 most-frequent events.
     % The training data comprises the top 10 events with most data and the remaining 105 events are utilized for testing. Intending to study the impact of event diversity on the zero-shot model performance, we create three training datasets by sampling a fixed 450 sentences\footnote{Fixing the training data size removes the confounding variable of data size for the study.} for $m$ events from the larger training corpus. We vary $m$ from 1 to 10 most-frequent events.
    \item Cross-type Transfer (CTT):
    % Adhering to the hierarchical event schema (refer to Appendix~\ref{sec:event-organization}), 
    We curate a training dataset comprising of events of a single abstraction category (e.g. Scenario), while the test dataset comprises events of all other abstraction types. This test suite also assesses models' transfer learning strength.
\end{itemize}

% For the zero-shot test suite, we select the top 10 events in terms of data availability as part of the training corpus and the remaining 105 events for the testing corpus.
% Intending to study the impact of event diversity on the zero-shot model performance, we create three training datasets by sampling a fixed 450 sentences\footnote{Fixing the training data size removes the confounding variable of data size for the study.} for $m$ events from the larger training corpus.
% We vary $m$ from 1 most-frequent event to 10 events.
% % Similar to limited data setting, we sample 5 different datasets and report the average model performance.
% The final test suite of cross-type transfer evaluates generalizability in terms of models' transfer learning strength.
% Adhering to the hierarchical event schema (refer to Appendix~\ref{sec:event-organization}), we curate a training dataset comprising of events of a single abstraction category (e.g. Scenario), while the test dataset comprises of events of all other abstraction types.

We report the data statistics for these benchmarking setups in Appendix~\ref{sec:data-statistics}.
For each of the test suites involving sampling, we sample 5 different datasets\footnote{All datasets will be released for reproducibility purpose.} and report the average model performance to account for the sampling variation.
% We believe that these different test suites can adequately evaluate the generalizability of the EAE models in various realistic scenarios.
% We use these different test suites to benchmark various EAE models (discussed in detail in Section~\ref{sec:results}).


\subsection{Models}
\label{sec:models}

% \ih{Remove DyGie++ for WQE}

% Traditional classification-based EAE models like OneIE \cite{lin-etal-2020-joint} and DyGIE++ \cite{wadden-etal-2019-entity} use a softmax to classify into the different argument roles.
% Using a softmax layer over 469 argument classes would be expensive and require good amounts of data per class for desirable discriminative training.
% Thus, we believe that the traditional classification based EAE models would perform poorly while scaling up to the large number of events in FN-115.
% On the other hand, QAEE \cite{du-cardie-2020-event} is a recent classification-based model which explores the use of label semantics by modeling event extraction as a question-answering task.

% \np{We cover wide and diverse set of baselines}
% We aim to evaluate the generalizability of various representative EAE models on our \dataName{} benchmarking test suites.
Overall, we benchmark six EAE models on our test suites. These models organized by their representative classes are described below. The implementation details are specified in Appendix~\ref{sec:implementation}.
% \tp{Mention Implementation details are in Appendix}
% \tp{@I-Hung, verify Query and Extract model here}

% \paragraph{Classification-based models:}
\mypar{Classification-based models:}
These traditional works predict arguments by learning to trace the argument span using a classification objective.
We experiment with three models, namely
(1) \textbf{DyGIE++} \cite{wadden-etal-2019-entity}, a traditional model utilizing multi-sentence BERT encodings and span graph propagation.
(2) \textbf{OneIE} \cite{lin-etal-2020-joint}, a multi-tasking objective-based model exploiting global features for optimization.
(3) \textbf{Query\&Extract} \cite{wang-etal-2022-query} utilizing the attention mechanism to extract arguments from argument role queries.

% \paragraph{Question-Answering models:}
\mypar{Question-Answering models:}
Several works here formulated event extraction as a question-answering or machine reading comprehension task.
We consider one such model
(4) \textbf{BERT\_QA} \cite{du-cardie-2020-event}, a BERT-based model leveraging label semantics using a question-answering objective.
In order to scale BERT\_QA to the wide range of argument roles, we generate question queries of the form ``\textit{What is \{arg-name\}?}'' for each argument role \textit{\{arg-name\}}.

% \paragraph{Generation-based models:}
\mypar{Generation-based models:}
Inspired from great strides in generation, recent works framed EAE as a generation task using a language-modeling objective for training.
We consider two such models for our benchmarking:
(5) \textbf{TANL} \cite{Paolini21tacl}, a multi-task language generation model which treats EAE as a translation task.
(6) \textbf{DEGREE} \cite{hsu2021degree}, an encoder-decoder framework which extracts event arguments using natural language input prompts.

\noindent \textit{Automating DEGREE}:
DEGREE requires human effort for manually creating natural language prompts and thus, can not be directly deployed for the large set of event types in \dataName.
In our work, we undertake efforts to scale up DEGREE by proposing a set of automated refinements.
The first refinement automates the event type description as ``\textit{The event type is \{event-type\}}" where \textit{\{event-type\}} is the input event type.
The second refinement automates the event template generation by splitting each argument into a separate self-referencing mini-template ``\textit{The \{arg-name\} is some \{arg-name\}}" where \textit{\{arg-name\}} is the argument role.
The final event-agnostic template is a simple concatenation of these mini-templates.
We provide an illustration and ablation of these automated refinements for DEGREE in Appendix~\ref{sec:autodegree-ablation}.
% \tp{Should we add figure for illustration?}
% \tp{Should we mention about the ACE ablation study for our modeling is shown in the appendix?}

\subsection{Evaluation Metrics}
\label{sec:eval-metrics}

% \looseness=-1
Following the traditional evaluation for EAE tasks, we report the \textbf{micro F1} scores for argument classification.
To encourage better generalization across wide range of events, we also use \textbf{macro F1} score that reports the average of F1 scores for each event type.
% A good macro-F1 score would indicate better generalization by the model.
% Furthermore, we also report the macro-F1 scores to highlight the average performance across different event types.
For the limited data test suites, we record a model performance curve, wherein we plot the F1 scores against the number of training instances.

% \tp{add motivation of macro F1 here.}

==> intro.tex <==
\section{Introduction}

Event Argument Extraction (EAE) aims at extracting structured information of event-specific arguments and their roles for events from a pre-defined taxonomy.
% Figure~\ref{fig:ee_example} provides an illustration of EAE for the event type \textit{Assistance}, where models are expected to extract the event-specific roles of \textit{Helper} as \textit{Russia}, \textit{Benefiter} as \textit{Iran}, and \textit{Goal} as \textit{construct a dam} from the sentence.
% EAE is fundamental for the task of event extraction and has been well-studied in the domain of Information Extraction \cite{sundheim-1992-overview, grishman-sundheim-1996-message}.
% EAE is a fundamental task for information extraction and has been studied for a long time \cite{sundheim-1992-overview, grishman-sundheim-1996-message}.
% \cite{sundheim-1992-overview, grishman-sundheim-1996-message} and has been elemental
EAE is an old topic \cite{sundheim-1992-overview} and elemental for a wide range of applications like building knowledge graphs \cite{10.1145/3366423.3380107}, question answering \cite{berant-etal-2014-modeling}, and various other NLP applications \cite{hogenboom2016survey, yang-etal-2019-interpretable}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/diversity-bar.pdf}
    \caption{Distribution of event types into various abstract event types for \dataName{}, ACE, ERE, RAMS, and WikiEvents datasets.
    We observe that \dataName{} is relatively more diverse than the other datasets.}
    \label{fig:ace-in-geneva}
    \vspace{-1em}
\end{figure}

Previous works usually assume the availability of extensive high-quality human annotations for training EAE models.
However, in practice, there is a wide range of diverse events that have zero annotation in existing datasets \cite{zhang-etal-2021-zero}.
Hence, recent works focusing on generalizable EAE have gained more attention \cite{huang-etal-2018-zero, lyu-etal-2021-zero, sainz-etal-2022-textual}.
These works utilize existing EAE datasets like ACE \cite{doddington-etal-2004-automatic}, and ERE \cite{DBLP:conf/aclevents/SongBSRMEWKRM15}
to benchmark the generalizability of the proposed models.
%In Figure~\ref{fig:ace-in-geneva}, we present the distribution of event types across various \textit{abstract event types} \cite{wang-etal-2020-maven} for these EAE datasets.
%We note how 
However, as is shown in Figure~\ref{fig:ace-in-geneva}, these datasets have limited diversity as they focus only on two abstract event types\footnote{Abstract event types are defined as the top nodes of the event ontology tree created by MAVEN \cite{wang-etal-2020-maven}.} of Action and Change.
The limited diversity and event-type coverage restrict the ability of the existing datasets to robustly evaluate the generalizability of EAE models.

% \kh{Just have two contributions. Makes the flow the better.}

Towards this end, we introduce \dataName{} (\textbf{G}eneralizability B\textbf{EN}chmarking Dataset for \textbf{EV}ent \textbf{A}rgument Extraction), a diverse EAE dataset covering a broad range of 115 event types spanning five abstract event types (Figure~\ref{fig:ace-in-geneva}) and 220 argument roles to evaluate the generalizability of EAE models.
%To ensure wide event coverage and diversity, we first construct a large and diverse EAE ontology.
% spanning a wide set of 179 event types and 362 argument roles \kh{Don't mention numbers here. Just mention GENEVA numbers}.
We start with constructing a large and diverse EAE ontology. 
% Creating such a large-scale diverse ontology
% % with diverse event types 
% from scratch requires a lot of time and expert knowledge.
% of semantics and linguistics \tp{This line can be removed/shortened}.
% To ensure wide coverage of event types, we follow MAVEN's \cite{wang-etal-2020-maven} approach to reference FrameNet \cite{baker-etal-1998-berkeley-framenet}, a semantic role labeling (SRL) dataset \kh{Might want to distinguish work from MAVEN} \ih{Just mention MAVEN, an event detection dataset}\tp{Should we add the term "diverse" to emphasize how transferring from SRL yields greater diversity in GENEVA}.
% , to initiate our ontology creation.
To reduce human effort on ontology creation, we exploit the shared properties between semantic role labeling (SRL) and EAE \violet{can we find citations to support this connection?} and leverage a diverse and comprehensive SRL dataset FrameNet \cite{baker-etal-1998-berkeley-framenet}, to build our EAE ontology.
% This transfer is not trivial and poses challenges as SRL is a fine-grained linguistically-driven task and EAE is a higher-level extractive task \tp{Does this line not give the idea or clarity?}.
Through exhaustive human expert annotations, we design mappings that transform the FrameNet schema to a large and diverse EAE ontology.
% We overcome these challenges through exhaustive human expert annotation and design transfer mappings for FrameNet.
% Utilizing these mappings, we merge and filter events and argument roles in FrameNet to derive our large and diverse EAE ontology.
% Next, we extensively study the relations between SRL and EAE, and through exhaustive human expert annotations, we design event type and argument role mappings for FrameNet. 
% \ih{Remove the sentence about "study" and make the sentence more about "Why SRL?" - Compress 276--295 and put here.}
% After ontology creation, we generate our dataset \dataName{} by performing a task transfer from SRL to EAE.
We then exploit these human-curated ontology mappings
% of event types and argument roles
to transfer FrameNet data for EAE and generate our dataset \dataName.
Finally, we perform a bunch of 
% cleaning steps \ih{remove cleaning word. Not adds value.} and 
human validation steps to ensure the high quality of our dataset.

% To improve model generalizability,
% With the goal of pushing the limit of generalizability for EAE,
% we introduce a new model \modelName{} which inherits the current state-of-the-art EAE model in low-resource regime --- \degree~\cite{hsu2021degree}.
% Like \degree, \modelName{} performs EAE via generating sentences that summarize all the event argument information using automated natural language prompts.
% On the other hand, \modelName{} enhances generalizability by introducing automated refinements to eliminate the human effort required for scaling up \degree{} to a wide range of events.
% We evaluate \modelName{} along with various other EAE models on the \dataName{} test suites and demonstrate that
% \modelName{} establishes a strong generalizability benchmark on these test suites.

% \violet{I feel the \textbf{goal} of this paper is still not crystal clear. Is our goal benchmark generalizability, and thus we construct \dataName, or is our goal construct a dataset, and use that dataset we can do many things including benchmark the generalizability of EAE models. There are subtle differences between the two and I believe we're doing 1, but the bridge sentence below does not have the transition flow to emphasize that this is our final and most important goal.}
%In order 

%We employ our diverse dataset 
\dataName{} enables us to benchmark and evaluate the generalizability of various EAE models.
We design four benchmarking test suites to assess the models' ability to learn from limited training data and generalize to unseen event types.
These test suites are distinctly different based on the training and test data creation --
(1) low resource, (2) few-shot, (3) zero-shot, and (4) cross-type transfer settings.
For benchmarking, we consider various kinds of EAE models - 
traditional classification-based models like OneIE, Query\&Extract, and DyGIE++, question-answering based models like BERT\_QA, generative approaches like TANL and DEGREE.
% traditional classification-based models like OneIE \cite{lin-etal-2020-joint} and DyGIE++ \cite{wadden-etal-2019-entity}, question-answering based models like BERT\_QA \cite{du-cardie-2020-event}, generative approaches like TANL \cite{Paolini21tacl} and DEGREE \cite{hsu2021degree}.
We also introduce new automated refinements to generalize and scale up the manual input prompts used in DEGREE to the wide range of events in \dataName.
Our experiments reveal that traditional classification-based approaches show poor generalization.
DEGREE performs the best across test suites and establishes a strong benchmark with upto $30$ F1 points over classification approaches.
We conclude that using generative approaches and exploiting label semantics heavily boost model generalizability.
\tp{Are these conclusions good/compelling?}
% generative models perform significantly better than other approaches in terms of EAE generalizability.
% \tp{modify this based on final results}
% \violet{again, would be nice to provide additional insights on strengths and weaknesses of existing models and promising future directions for model design.}

% With the goal of pushing the limit of generalizability for EAE,
% we introduce a new model \modelName{} which inherits the current state-of-the-art EAE model in low-resource regime --- \degree~\cite{hsu2021degree}.
% Like \degree, \modelName{} performs EAE via generating sentences that summarize all the event argument information using automated natural language prompts.
% On the other hand, \modelName{} enhances generalizability by introducing automated refinements to eliminate the human effort required for scaling up \degree{} to a wide range of events.
% We evaluate \modelName{} along with various other EAE models on the \dataName{} test suites and demonstrate that
% \modelName{} establishes a strong generalizability benchmark on these test suites.

% To improve model generalizability, we introduce \modelName{}
% which inherits the current state-of-the-art EAE model in low-resource regime --- \degree~\cite{hsu2021degree}.
% \modelName{} performs EAE via generating sentences that summarize all the event argument information using automated natural language prompts. %which helps in scaling up to a wide range of event types and argument roles.
% \modelName{} achieves better generalizability compared to traditional classification-based EAE models as it leverages label semantics when making predictions owing to the automated natural language prompts.
% On the other hand, the automated refinements in \modelName{} help eliminate the human effort required for scaling up \degree{} to the wide range of events.
% Overall, \modelName{} establishes a strong benchmark on the \dataName{} test suites, as we will show in Section~\ref{sec:results}.

To sum up, we make the following contributions. We construct a large and diverse EAE ontology by transferring an SRL dataset FrameNet for EAE. Using this ontology, we create a diverse EAE dataset \dataName{} spanning 115 event types from 5 abstract domains and 220 argument roles. To test the different aspects of the generalizability of EAE models, we design four benchmarking test suites. Finally, we conduct a thorough evaluation of various EAE models on these test suites in \dataName{} and provide key insights for improving model generalizability.


==> model.tex <==
\section{Proposed Model --- \modelName}

% \ih{Title: Methodology. 5.1 - Baseline models - have a couple of paragraphs about the shortcomings of previous methods and introduce DEGREE. Include the need of automation.
% 5.2 - Introduce DAM and the automation}

% \begin{itemize}
%     \item Large number of events. Fewer datapoints per event. Classification models suffer.
%     \item We look at generative models - specifically DEGREE. Challenges still involved as it's not 100\% automated.
% \end{itemize}

% We first discuss some background about previous EAE models and their applicability with respect to FN-115.
% We then introduce our model - \modelName in the later part of the section.
% \kh{Introduce generative models and subtly introduce DEGREE}
% \ih{Talk about advantages and abilities of SCAD here. Later mention how it's based on DEGREE.}
% In order to generalize on \dataName, we propose a new model \modelName.
In our work, we introduce a new model \modelName{} which aims to provide better generalizability for EAE.
\modelName{} reforms a recent approach \degree~\cite{hsu2021degree} with automated refinements.
These refinements aid \modelName{} to scale up robustly to a wide range of event types while eliminating the human effort requirements of \degree.
% which has shown superior performance in the low-data regime.
In this section, we first briefly introduce the base \degree{} model and then describe our proposed model \modelName.

\subsection{\degree}

% \ih{Move relevant portions to related work in Section 2}

% \subsection{Baseline Models}

% As observed in Table~\ref{tab:dataset-coverage}, there are fewer mentions per event type in FN-115.
% Thus, there is a need for good generalizability and the ability to learn from less data for the models to perform well on FN-115.
% Traditional classification-based EAE models use a softmax to classify into the different argument roles, which is an expensive and data-hungry operation.
% We rather move towards the recently introduced generation-based approaches which have proven to be more generalizable.

% With the broad range of events and the dense nature of mentions per sentence, there are fewer datapoints per event type in \dataName.
% Thus, scaling up performance for FN-115 really requires a good generalizability in models to learn from fewer datapoints.
% Traditional classification-based EAE models like OneIE \cite{lin-etal-2020-joint} and DyGIE++ \cite{wadden-etal-2019-entity} use a softmax to classify into the different argument roles.
% Using a softmax layer over 469 argument classes would be expensive and require good amounts of data per class for desirable discriminative training.
% Thus, we believe that the traditional classification based EAE models would perform poorly while scaling up to the large number of events in FN-115.
% On the other hand, QAEE \cite{du-cardie-2020-event} is a recent classification-based model which explores the use of label semantics by modeling event extraction as a question-answering task. \tp{End of para needs some check.}

% \np{Don't introduce the other baselines and talk about them in the experimental setup. Briefly introduce or compare degree to previous methods.}

% \degree{}\footnote{For our work, we consider the EAE version of DEGREE.} \cite{hsu2021degree} is a recently proposed EAE model and has shown superior performance in the low-data regime.
\degree{}\footnote{For our work, we consider the EAE version of \degree.} is an encoder-decoder based generative model which 
% \degree{}\footnote{For our work, we consider the EAE version of \degree.} 
utilizes natural language templates as part of input prompts.
The input prompt comprises of three components - (1) \textit{Event Type Description} which provides a definition of the given event type, (2) \textit{Query Trigger} which indicates the trigger word for the event mention, and (3) \textit{EAE Template} which is a natural sentence combining the different argument roles of the event.
% DEGREE\footnote{For our work, we consider the EAE version of DEGREE.} utilizes natural sentence templates as part of prompts to extract argument roles.
Conditioned on the input prompt, the model generates a natural language sentence with the extracted arguments.
Restructuring argument roles into natural language input prompts helps \degree{} better leverage label semantics, and this fundamentally assists it to generalize in the low-data setting.
% It remodels the structured EAE outputs (i.e. argument roles) into natural language sentences to better leverage the pre-training language modeling objective, and this fundamentally helps the model generalize faster.
% The argument roles are finally extracted from the generated output text.
We illustrate \degree{} along with an example of its input prompt design in Figure~\ref{fig:degree-eae}.
% Generative models have shown great performance gains for classification \cite{schick-schutze-2021-exploiting, schick-schutze-2021-just} and have been explored for structured prediction as well.
% These approaches convert the structured output into a natural text sentence to better leverage the language modeling pre-training objective, and thus can generalize faster.
% One of the many generative approaches is \degree \cite{hsu2021degree} which has shown robust performance in few-shot settings.
% \degree\footnote{For our work, we only consider the EAE version of DEGREE.} is a generative model which utilizes natural sentence templates as part of prompts to extract argument roles.
% It is essentially an encoder-decoder architecture that uses a passage-prompt combination as input to generate an output natural text (as shown in the top half of Figure~\ref{fig:degree-eae}).

% We provide an illustration of each of these three components in the bottom half of Figure~\ref{fig:degree-eae}.
% \tp{Add more technical description of DEGREE?}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/manual-prompt.pdf}
    \caption{Model architecture of \degree{} (top half) and an illustration of a manually created prompt for the event type \textit{Employment} (bottom half).
    }
    \label{fig:degree-eae}
    \vspace{-0.7em}
\end{figure}

% Although \degree performs well in zero-shot and few-shot setting, it requires manual human effort for creation of templates and event descriptions for each event type.
% This would not be scalable for FN-115 as the dataset has 115 unique event types and 450+ unique arguments.
% Although \degree performs well in zero-shot and few-shot setting, it cannot be applied to \dataName directly.
Despite the superior performance of \degree{} in the low-data setting, it can not be deployed on \dataName{}.
This is because \degree{} requires manual human effort for the creation of input prompts for each event type and argument role and can't be scaled to 115 event types and 187 argument roles in \dataName.
% This would not be scalable as \dataName{} has 115 event types and 187 argument roles.
Thus, there is a need to automate the manual human effort to scale up \degree.
% to a broad range of new events.
% We introduce a new model DAM, which uses the same working principle of \degree to utilize natural language prompts while completely automating various manual components of DEGREE.
% We describe this new automated \degree model in the next subsection.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/automated-prompt.pdf}
    \caption{An illustration of an automatically generated prompt by \modelName{} for the event type \textit{Employment}.}
    \label{fig:automated-prompt}
    \vspace{-0.7em}
\end{figure}

\subsection{\modelName}
\label{sec:dam}

% \ih{Emphasize how we don't change the working principle (natural sentences), but make adaptations to scale-up to wide-range of arguments.}
\modelName{} exploits the same working principle of using natural language input prompts as \degree, while scaling up the prompt creation pipeline via automated refinements.
\degree{} requires human effort for two input prompt components - (1) Event Type Description and (2) EAE Template.
% DAM uses simple heuristics to automate these two components, which we describe below.
We describe the automated refinements in \modelName{} for these components below.

\subsubsection{Automating Event Type Description}
Event type description is a natural language sentence describing the event type.
In order to automate this component, we propose a simple heuristic that creates a simple natural language sentence mentioning the event type - ``\textit{The event type is \{event-type\}}".
% Since the event name is available as part of the input, generating this description is easy to automate.
, as illustrated in Figure~\ref{fig:automated-prompt}.
% In order to automate, we propose two heuristics -
% (1) No description, and
% (2) Event Type Mention.
% The first one completely removes the event type description from the prompt.
% The second heuristic creates a natural language while only mentioning the event type.
% % Since the event name is available as part of the input, generating this description is easy to automate.
% \modelName{} utilizes the second heuristic and we show an illustration of the same in Figure~\ref{fig:automated-prompt}.

\subsubsection{Automating EAE Template}
EAE template generation in \degree{} can be split into two subtasks, which we discuss in detail below.

% \paragraph{Argument Role Mapping:}
\mypar{Argument Role Mapping:}
This subtask maps each argument role to a natural language placeholder phrase based on the characteristics of the argument role.
For example, the argument role \textit{Employer} is mapped to ``\textit{some organization}'' in Figure~\ref{fig:degree-eae}.
While training, \degree{} learns to replace these placeholders in the prompt with the arguments from the passage.
Mapping each unique argument role to a placeholder phrase requires commonsense knowledge, and thus rendering this subtask manual in nature.
% For automating this mapping, we need to find an appropriate phrase for each new argument role encountered.

For automating this mapping process, we propose a simple refinement of self mapping.
% Default mapping maps each argument role to a default placeholder phrase ``\textit{something}''.
Self mapping maps each argument role to a self-referencing placeholder phrase ``\textit{some \{arg-name\}}'', where \textit{\{arg-name\}} is the argument role itself.
For example, the argument role \textit{Employer} would be mapped to ``\textit{some employer}''.
We illustrate an example of this heuristic in Figure~\ref{fig:automated-prompt}.

% For automating this mapping process, we propose two refinements - (a) Default mapping, and (b) Self mapping.
% Default mapping maps each argument role to a default placeholder phrase ``\textit{something}''.
% Self mapping maps each argument role to a placeholder phrase ``\textit{some \{arg-name\}}'', where \textit{\{arg-name\}} is the argument role.
% For example, the argument role \textit{Employer} would be mapped to ``\textit{some employer}''.
% \modelName{} utilizes self mapping for automating this subtask, as illustrated in Figure~\ref{fig:automated-prompt}.

% \paragraph{Template Generation:}
\mypar{Template Generation:}
The second subtask requires generating a natural sentence(s) using the argument role mapped placeholder phrases (as shown in Figure~\ref{fig:degree-eae}).
Each event type comprises of a distinct set of argument roles.
Thus, generating EAE templates for each event type is tedious and created by human in \degree{}.
% Each event is associated with a different action and a unique structure for how argument roles interact with each other.
% Thus, generating a natural language sentence encompassing all different argument roles would be a tedious and manual task.
% Each event would have a unique natural language sentence depending on the structure of the event and its arguments.

% In order to automate this subtask, we create an event-agnostic template which would function well for any new event structures.
In order to automate this subtask, \modelName{} utilizes an event-agnostic template composed of argument role-specific sentences.
For each argument role in the event, we generate a sentence of the form ``\textit{The \{arg-name\} is \{arg-map\}.}'' where \textit{\{arg-name\}} and \textit{\{arg-map\}} is the argument role and its mapped placeholder phrase respectively.
For example, the sentence for argument role \textit{Employer} with self mapping would be "\textit{The employer is some employer.}".
The final event-agnostic template is a simple concatenation of all the argument role sentences.
We provide an illustration of the event-agnostic template in Figure~\ref{fig:automated-prompt}.



==> old-old-results.tex <==
\section{Results and Analysis}
\label{sec:results}

\tp{Needs a change}
Similar to the benchmarking setups discussed in Section~\ref{sec:benchmark-setup}, we organize the main experimental results into limited training data and no training data settings.
Later we show an analysis of macro-F1 score performance of the different models and finally provide an ablation study for the \modelName model.

% We evaluate the generalizability of various models and present the results in the few-shot and zero-shot benchmarking setups (as described in Section~\ref{sec:benchmark-setup}).
% Later, we show the impact of the various automation heuristics used in \modelName by an ablation study.

% \ih{Classify into two categories - (1) LR and FS in limited-data and (2) ZS and DA. Find appropriate names to both.}

% \kw{Expand on the summary above and some key questions we are analyzing. Tie it to generalizability in intro.}

\subsection{Limited Training Data}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/low-res-results.pdf}
    \caption{Model performance in micro-F1 scores against the number of training event mentions (log-scale) for the low-resource test suite.
    \tp{Should I change this to matplotlib?}
    \np{Increase fontsize for things}
    % \kw{Add different line styles for color-blind and black-white figures.}
    % \kw{Write key observation in caption.}
    }
    \label{fig:random_sampling_micro_f1}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/few-shot-results.pdf}
    \caption{Model performance in micro-F1 scores against the number of training event mentions per event for the few-shot test suite.
    % \tp{Dummy figure for uniform sampling}.
    % \kw{Observations from macro F1 scores are similar.}
    }
    \label{fig:uniform_sampling_micro_f1}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/lr-micro-nopre.pdf}
%     \caption{Model performance in micro-F1 scores against the number of training event mentions (log-scale) for the low-resource test suite.
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     }
%     \label{fig:lr_micro_f1}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/lr-macro-nopre.pdf}
%     \caption{Model performance in macro-F1 scores against the number of training event mentions (log-scale) for the low-resource test suite.
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     }
%     \label{fig:lr_micro_f1}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/fs-micro-nopre.pdf}
%     \caption{Model performance in micro-F1 scores against the number of training event mentions per event for the few-shot test suite.
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     }
%     \label{fig:lr_micro_f1}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/fs-macro-nopre.pdf}
%     \caption{Model performance in macro-F1 scores against the number of training event mentions per event for the few-shot test suite.
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     }
%     \label{fig:lr_micro_f1}
% \end{figure}

% \paragraph{Random Sampling}
Limited training data setting comprises of the low resource and the few-shot test suites.
We present the results for the model performance in terms of micro-F1 scores for these test suites in Figure~\ref{fig:random_sampling_micro_f1} and Figure~\ref{fig:uniform_sampling_micro_f1} respectively.
% \footnote{We present the complete set of results in the Appendix.}.
% We present the results for the model performance in terms of micro-F1 score in the few-shot setup with random sampling and uniform sampling in Figure~\ref{fig:random_sampling_micro_f1} and Figure~\ref{fig:uniform_sampling_micro_f1} respectively\footnote{We present the complete set of results in the Appendix.}.
% OneIE and DyGie++ achieve a model performance of $38.84$ and $35.5$ \tp{update number} respectively when trained on complete data.
When trained on complete training data (rightmost point in Figure~\ref{fig:random_sampling_micro_f1}), we observe that DyGIE++ performs the best with an F1-score of $66.62$, while \modelName and QAEE follow closely.
On the other hand, OneIE achieves a poor F1-score of $38.84$ which can be attributed to its model design and the inability to deal with overlapping argument roles.
Due to this inferior performance, we do not compare OneIE to the model performance curves in the figures.
% Furthermore, the observed trends are similar for macro-F1, hence we do not show them in the figures.

Across all sampling scenarios in the low resource and few-shot test suites, we observe that the \modelName model outperforms all other models significantly.
% From the figures, we observe that when models are trained from scratch (the solid lines), \modelName performs significantly better on all sets of training event mentions.
This holds true when the models are trained from scratch (the solid lines) as well as when the models are fine-tuned from their ACE pre-trained versions (the dashed lines).
% This trend also follows when the models are pre-trained on the ACE dataset.
This demonstrates the superior generalizability of \modelName (and generally generative approaches) over the other approaches.
On the other hand, DyGIE++ which is a traditional classification approach performs well only in the high data setting and exhibits poor performance in the low-data setting.

From both the figures, we observe that pre-training the model on the ACE dataset improves the model performance (compared to training from scratch), especially when the training data size is low.
But the zero-shot performance (leftmost point in both figures) is rather limiting with $12.83$ for \modelName and $6.32$ for QAEE.
Thus, it's not trivial to transfer significant model performance from ACE to \dataName.
This indicates how \dataName is distinctively more challenging than the standard ACE dataset.

\subsection{No Training Data}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/zero-shot-results-bar.pdf}
    \caption{Model performance in micro-F1 scores across different number of training event types (while keeping the amount of training data constant) for the zero-shot test suite.
    % \ih{Convert to stacked bar graph}
    }
    \label{fig:zero-shot-benchmarking}
\end{figure}

\begin{table}[t]
    \centering
    \begin{tabular}{l|rr|rr}
        \toprule
        & \textbf{\modelName} & \textbf{+PT} & \textbf{QAEE} & \textbf{+PT} \\
        \midrule
        CTT & 27.26 & 33.09 & 7.83 & 16.29 \\
        \bottomrule
    \end{tabular}
    \caption{Model performance in micro-F1 scores for the cross-type transfer (CTT) test suite. Here, +PT indicates model performance when the model is pre-trained on the ACE dataset.}
    \label{tab:ctt-results}
\end{table}

This data setting includes the zero-shot and the cross-type transfer test suites.
Traditional models like DyGIE++ and OneIE cannot support unseen events or argument roles and thus, we do not include them in the experiments for this data setting.
% \tp{comment about DyGIE and OneIE}

We show the model performance for \modelName and QAEE in the zero-shot test suite in Figure~\ref{fig:zero-shot-benchmarking}.
Similar to the limited data setting, \modelName outperforms the other models and establishes its better generalizability.
We further observe performance gains for all models as we increase the number of events in the training data (while keeping the training data size constant).
On the other hand, these gains reduce as the number of training events increases.
Thus, we conclude that event diversity helps improve zero-shot performance but provides marginally reducing gains.
% \tp{plot for zero-shot and numbers in table for cross-type transfer}

We present the results for the cross-type transfer test-suite in Table~\ref{tab:ctt-results}.
We observe that the \modelName shows great transfer capabilities as it outperforms the QAEE model by a significant margin.
The training data for this test suite comprises of all data for 9 events from the Scenario abstraction type (refer to Appendix~\ref{sec:event-organization}).
Despite having a good amount of event diversity, we observe that the model performance is poorer for this test suite than the zero-shot test suite with similar number of events.
This highlights the additional challenge of transferring across different event types introduced by this test suite.

% We also observe that the pre-trained models outperform their respective models trained from scratch.
% The performance gains reduce as the number of training datapoints increase.
% This underlines how pre-training helps in better domain adaptation, and more especially in the low-resource setting.

% From the figures, we observe that when models are trained from scratch, \modelName outperforms other baseline models significantly on all sets of training event mentions.
% This trend also follows when the models are pre-trained on the ACE dataset.
% This highlights the generalizability and superior performance of \modelName (and generally generative approaches) over classification-based approaches.

% We also observe that the pre-trained models outperform their respective models trained from scratch.
% The performance gains reduce as the number of training datapoints increase.
% This underlines how pre-training helps in better domain adaptation, and more especially in the low-resource setting.

% \kw{Use three different figures to highlight individual aspects.}

% \paragraph{Uniform Sampling}
% In this setup, we uniformly sample equal number of event mentions per event and show the model performance results for micro-F1 in Figure~\ref{fig:uniform_sampling_micro_f1}.
% Similar to random sampling, we observe how \modelName outperforms other baseline models and also how pre-training helps improve model performance significantly.

% Overall, the best model F1 score with full training (the points on the extreme right) is still around 60 in Figure~\ref{fig:random_sampling_micro_f1}.
% This shows how \dataName is a challenging dataset and there is a large scope for overall improvement.

\begin{table}[t]
    \centering
    \begin{tabular}{lrrrr}
        \toprule 
        Model & LR & FS & ZS & CTT \\
        \midrule
        % OneIE & & \\
        DyGIE++ & -4.56 & \textbf{1.02} & - & - \\
        QAEE & -4.31 & -3.28 & -2.69 & -0.64 \\
        \modelName & \textbf{-2.36} & -1.45 & \textbf{-0.62} & \textbf{-0.1}\\
        \bottomrule
    \end{tabular}
    \caption{Average difference between the macro-F1 and micro-F1 scores for the models in the different benchmarking test suites. LR = low resource, FS = few-shot, ZS = zero-shot, and CTT = cross-type transfer.
    % \tp{Add standard deviation as well if it's significant to show}
    }
    \label{tab:macro-f1-difference}
\end{table}

\subsection{Macro-F1 Analysis}

Naturally, the trends of the model performance are similar across micro-F1 and macro-F1 scores and might not provide additional insights.
Instead, we study the difference between the macro-F1 and the micro-F1 scores.
A high difference (face value and not absolute terms) indicates a more uniform performance across all events and lesser bias towards events with higher data, which in turn, establishes better generalizability.
We present the average difference between the scores for different models across different test suites in Table~\ref{tab:macro-f1-difference}.

% In order to study the macro-F1 model performance, we show the average difference between the macro-F1 and micro-F1 scores of the different models in both the data setups in Table~\ref{tab:macro-f1-difference}.
% A low macro-F1 score (or a highly negative difference) indicates a poor uniform performance across all event types which would be due to the bias of event types with higher datapoints.
% We observe that the difference is negative most cases, which indicates that the micro-F1 is better than the macro-F1 scores.

% \tp{This para will change according to results}
Although DyGIE++ has a high positive difference in the few-shot setting, its absolute micro-F1 scores are super poor (as seen in Figure~\ref{fig:uniform_sampling_micro_f1}).
Overall, we observe that \modelName has the highest difference across most benchmarking test suites.
% We observe that in both sampling setups, the absolute difference is much lesser for \modelName compare to the other models.
This emphasizes how \modelName generalizes uniformly across all event types.
% We also observe a better difference in uniform sampling compared to random sampling setup.
% This indicates how uniform sampling presents a good benchmarking test suite to evaluate the generalized model performance across all events.
Across the different benchmarking suites, we observe that the difference is more in the no training data setting (ZS and CTT) compared to the limited training data setting (LR and FS).
This disparity shows how training data can bias the models towards certain event types and hinder uniform model performance.
% \tp{Conclusion for previous observation. Overall, need a better table/conclusion for this part.}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/random-sampling-micro-f1.png}
%     \caption{Macro-F1 score distribution of the best trained models.}
%     \label{fig:macro-f1-distribution}
% \end{figure}

% \tp{We might add another paragraph to discuss the distribution of F1 scores between the models.}

% \subsection{Zero-shot Benchmarking}

% We show the main results for zero-shot benchmarking in Figure~\ref{fig:zero-shot-benchmarking}.
% Note that we used a fixed amount of training data while varying the number of training events.
% First, we observe that the \modelName outperforms the QAEE baseline significantly and shows good generalization even in the zero-shot setting.
% Secondly, we observe that the model performance difference doesn't vary significantly as we increase the number of events in the training data.
% This indicates that for the same amount of training data, increasing event diversity doesn't improve the performance much.
% \tp{Comment about model performance and pre-training}
% \ih{Need to add a bunch of other baselines for zero-shot claim}

% \tp{Paragraph and comments about how diversity of many event types affects model performance.}

% \subsection{Ablation Study of \modelName with \degree}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lr}
%         \toprule
%         & Micro-F1 \\
%         \midrule
%         DEGREE & 57.46 \\
%         \midrule
%         \quad w/ no event description & 57.32 \\
%         \quad w/ event type mention & 57.45 \\
%         \midrule
%         \quad w/ default mapping & 54.18 \\
%         \quad w/ argument mapping & 56.04 \\
%         \midrule
%         \quad w/ event-agnostic template & 59.04 \\
%         \midrule
%         \modelName & 56.62 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Ablation results for various automation heuristics experimented for automating the \degree model on the \ablationDataName dataset.}
%     \label{tab:automation-ablation}
% \end{table}

% As discussed in Section~\ref{sec:dam}, we introduce simple heuristics to automate the various manual components in prompt generation in the \degree model.
% % In order to evaluate the impact of these heuristics, we ablate each of these heuristics individually and compare them with model performance using the \degree model.
% Here, we provide an ablation study for each of these heuristics to evaluate their individual impact on the model performance.
% % We need to manually write descriptive prompts for each event type for the original \degree model.
% Since \degree requires manual annoation for each event type, we sample a small dataset \ablationDataName comprising of 10 event types from the original 
% We introduce a smaller dataset \ablationDataName comprising of 10 event types from the original FrameNet dataset for this ablation.
% We show these ablation results on the \ablationDataName dataset in Table~\ref{tab:automation-ablation}.

% First, we observe that automating event type description using no description or event type mention (second and third rows) yields very little performance difference.
% The major performance drop happens when automating argument role mapping and the corresponding results are shown in the fourth and fifth rows respectively.
% Surprisingly, we observe that replacing the original template with an event-agnostic template leads to an improvement in the performance.
% Overall, when we combine all these individual heuristics to get the \modelName model, we observe less than 1 point of F1 score dip.
% Thus, we show that \modelName scales up \degree while providing nearly similar performance.
% % \tp{Paragraph describing not much performance dip. Also write about ACE pre-training and comparable results there as well.}

% \subsection{Pre-training experiments}

% \tp{ACE v/s ERE v/s ACE-ERE}

==> rel_works.tex <==
\section{Related Work}

% \tp{Need to reduce this section}

% \paragraph{Event Extraction Datasets}
\mypar{Event Extraction Datasets:}
The earliest datasets in event extraction date back to MUC \cite{sundheim-1992-overview, grishman-sundheim-1996-message}.
Later ACE \cite{doddington-etal-2004-automatic} was introduced and is one of the most used datasets.
The ACE event schema is further simplified and extended to ERE \cite{DBLP:conf/aclevents/SongBSRMEWKRM15}.
ERE was later used to create various TAC KBP Challenges \cite{ellis2014overview, ellis2015overview, getman2017overview}.
These datasets cover a small number of event types and argument roles with limited diversity, and thus, can't be utilized to adequately evaluate the generalizability of EAE models.
MAVEN \cite{wang-etal-2020-maven} introduced a massive and diverse dataset spanning a wide range of event types.
However, the applicability of this dataset is limited to the task of Event Detection\footnote{Event Detection aims at only identifying the event type documented in the sentence.} and it does not contain argument annotations.
Recent works have introduced datasets like RAMS \cite{ebner-etal-2020-multi}, WikiEvents \cite{li-etal-2021-document}, and DocEE \cite{tong-etal-2022-docee}; but their diversity is also restricted to specific abstract event types
% and covers much less and diverse set of event types and argument roles,
as shown in Figure~\ref{fig:ace-in-geneva}.
Furthermore, these datasets are built with a focus on document-level event extraction, while in our work, we consider EAE at the sentence level.

% \paragraph{Event Argument Extraction Models}
\mypar{Event Argument Extraction Models:}
Traditionally, EAE has been formulated as a classification problem \cite{nguyen-etal-2016-joint-event}.
Previous classification-based approaches have utilized pipelined approaches \cite{yang-etal-2019-exploring, wadden-etal-2019-entity} as well as incorporating global features for joint inference \cite{li-etal-2013-joint, yang-mitchell-2016-joint, lin-etal-2020-joint}.
However, most of these classification approaches are data-hungry and do not generalize well in the low-data setting \cite{liu-etal-2020-event, hsu2021degree}.
To improve generalizability, some works have explored better usage of label semantics by formulating EAE as a question-answering task \cite{liu-etal-2020-event, li-etal-2020-event, du-cardie-2020-event}.
Recent approaches have explored the use of natural language generative models for classification and structured prediction for better generalizability \cite{schick-schutze-2021-exploiting, schick-schutze-2021-just}.
TANL \cite{Paolini21tacl} treats EAE as a translation between augmented languages, whereas Bart-Gen \cite{li-etal-2021-document} is another generative approach that focuses on document-level EAE.
\degree~\cite{hsu2021degree} is a recently introduced state-of-the-art generative model which has shown better performance in the limited data regime.
Another set of works transfer knowledge from similar tasks like abstract meaning representation and semantic role labeling \cite{huang-etal-2018-zero, lyu-etal-2021-zero, zhang-etal-2021-zero} to perform EAE. \looseness=-1
% Various works have also explored approaches for zero-shot transfer learning \cite{huang-etal-2018-zero, lyu-etal-2021-zero, zhang-etal-2021-zero}.
% \ih{Low-resource and generalizable models} \tp{Does it seem better now? Do we need to handle why we don't show them in our experiments here?}

% Due to the limitation of prior benchmarking datasets, it is unclear if these approaches can be generalized to handle a diverse set of events.
Since the evaluation of these models is done on previous EAE datasets, it is unclear if these approaches can be generalized to handle a diverse set of events.
In our work, we benchmark various classes of previous models on our dataset.
% Furthermore, we propose a new model \modelName{} which outperforms previous models and serves as a strong baseline for future works.
% In our work, we build upon one of the generative approaches to present a scalable model for EAE. 


==> results.tex <==
\section{Results and Analysis}
\label{sec:results}

Following \S~\ref{sec:benchmark-setup}, we organize the main experimental results into limited training data and unseen event data settings.
When trained on complete training data, we observe that 
OneIE and Query\&Extract achieve poor micro F1 scores of just $30.03$ and $40.41$ while all other models achieve F1 scores above $55$.
This can be attributed to the model designs of these models as they are unable to handle overlapping arguments.\footnote{One key attribute of \dataName{} is that arguments overlap with each other quite frequently in a sentence.}
Due to their inferior performance, we do not include OneIE and Query\&Extract in the benchmarking results.
We present the full results in Appendix~\ref{sec:all-results}.
% \sdl{I think if this is the case then we probably can restructure 5.1. to exclude OneIE's detailed description, and we simply say "we also investigate the performance of OneIE, which is bla bla. However, we find OneIE fails to achieve comparable results with other baselines, thus blablabla; but the current one is also OK to me.}

% Later we show an analysis of macro-F1 score performance of the different models and finally provide an ablation study for the \modelName model.

% We evaluate the generalizability of various models and present the results in the few-shot and zero-shot benchmarking setups (as described in Section~\ref{sec:benchmark-setup}).
% Later, we show the impact of the various automation heuristics used in \modelName by an ablation study.

% \ih{Classify into two categories - (1) LR and FS in limited-data and (2) ZS and DA. Find appropriate names to both.}

% \kw{Expand on the summary above and some key questions we are analyzing. Tie it to generalizability in intro.}

\subsection{Limited Training Data}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/low-res-results.pdf}
%     \caption{Model performance in micro-F1 scores against the number of training event mentions (log-scale) for the low-resource test suite.
%     \tp{Should I change this to matplotlib?}
%     \np{Increase fontsize for things}
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     }
%     \label{fig:random_sampling_micro_f1}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/few-shot-results.pdf}
%     \caption{Model performance in micro-F1 scores against the number of training event mentions per event for the few-shot test suite.
%     % \tp{Dummy figure for uniform sampling}.
%     % \kw{Observations from macro F1 scores are similar.}
%     }
%     \label{fig:uniform_sampling_micro_f1}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/lr-micro-nopre.pdf}
%     \caption{Model performance in micro-F1 scores against the number of training event mentions (log-scale) for the low resource test suite.
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     }
%     \label{fig:lr_micro_f1}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/lr-macro-nopre.pdf}
%     \caption{Model performance in macro-F1 scores against the number of training event mentions (log-scale) for the low resource test suite.
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     \tp{Will converge Figure 6 and 7 into a single one}
%     \np{Show macro first if results are better.}
%     }
%     \label{fig:lr_macro_f1}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/fs-micro-nopre.pdf}
%     \caption{Model performance in micro-F1 scores against the number of training event mentions per event for the few-shot test suite.
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     }
%     \label{fig:fs_micro_f1}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/fs-macro-nopre.pdf}
%     \caption{Model performance in macro-F1 scores against the number of training event mentions per event for the few-shot test suite.
%     % \kw{Add different line styles for color-blind and black-white figures.}
%     % \kw{Write key observation in caption.}
%     \tp{Will converge Figure 8 and 9 into a single one}
%     }
%     \label{fig:fs_macro_f1}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/lr-both-results.pdf}
    \caption{
    \looseness=-1
    Model performance in macro F1 (top) and micro F1 (bottom) scores against the number of training event mentions (log-scale) for the low resource suite.
    % \kw{Add different line styles for color-blind and black-white figures.}
    % \kw{Write key observation in caption.}
    }
    \label{fig:lr_results}
    \vspace{-3mm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/fs-both-results.pdf}
    \caption{Model performance in macro F1 (top) and micro F1 (bottom) scores against the number of training event mentions per event for the few-shot suite.
    % \kw{Add different line styles for color-blind and black-white figures.}
    % \kw{Write key observation in caption.}
    }
    \label{fig:fs_results}
    \vspace{-3mm}
\end{figure}

% Limited training data setting comprises of the low resource and the few-shot test suites.
% We present the model benchmarking results in terms of macro F1 and micro F1 scores for the low resource test suite in Figure~\ref{fig:lr_results}.
% We observe that \modelName{} beats all other baselines significantly in terms of macro F1 and performs well uniformly across all event types.
% Although TANL and DyGIE++ achieve high micro F1 when trained on high number of training instances, their macro scores are still relatively poor.
% This indicates that these models are biased towards specific events and do not generalize well.

% In Figure~\ref{fig:fs_results}, we show the benchmarking results on the few-shot test suite.
% The results showcase the clear hierarchy of the model performance, wherein \modelName{} significantly outperforms all other models.
% We also observe the poor performance of traditional classification-based approaches like DyGIE++ and this underlines the importance of using label semantics for better generalizability.
% % Overall, these results demonstrate the superior generalizability of \modelName (and generally generative approaches) over the other approaches.

Limited training data setting comprises of the low resource and the few-shot test suites.
We present the model benchmarking results in terms of macro F1 and micro F1 scores for the low resource test suite in Figure~\ref{fig:lr_results} and for the few-shot test suite in Figure~\ref{fig:fs_results}.
We observe that \modelName{} outperforms all other models significantly
% in terms of both F1 scores
for both the test suites and shows superior generalizability.
In general, we observe that generative-based models like DEGREE and TANL show better generalization and perform better than other model variants.
We also detect a stark drop from micro to macro F1 scores for TANL and DyGIE++ in the low resource test suite.
This indicates that these models are more easily biased towards specific events and do not generalize well uniformly.
We also observe the poor performance of traditional classification-based approaches like DyGIE++ and this underlines the importance of using label semantics for better generalizability.

\subsection{Unseen Event Data}

This data setting includes the zero-shot and the cross-type transfer test suites.
We collate the results in terms of micro F1 scores
% \footnote{Macro F1 performance results reported in Appendix~\ref{sec:macro-unseen}} 
for both the test suites in Table~\ref{tab:no-train-results}.
Models like DyGIE++ and TANL cannot support unseen events or argument roles
and thus, we do not include these models in the experiments for these test suites.

From Table~\ref{tab:no-train-results}, we observe that \modelName{} achieves the best scores across both test suites outperforming BERT\_QA by a significant margin of almost $13$-$15$ F1 points.
% Furthermore, for the cross-type transfer, we observe that the \modelName{} outperforms BERT\_QA by a significant margin of almost $20$ F1 points.
This establishes the superior transferability of \modelName{} to unseen event types and argument roles.
% We also record performance gains for both models as we increase the number of events in the training data.
% On the other hand, these gains reduce as the number of training events increases.
% Thus, we conclude that event diversity helps improve zero-shot performance.
% but provides marginally reducing gains.

\begin{table}[t]
    \centering
    \small
    % \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l|rrr|r}
        \toprule
        \textbf{Model} & \textbf{ZS-1} & \textbf{ZS-5} & \textbf{ZS-10} & \textbf{CTT} \\
        \midrule
        BERT\_QA & 5.05 & 21.53 & 24.24 & 11.17 \\
        \modelName & \textbf{24.06} & \textbf{34.68} & \textbf{39.43} & \textbf{27.9} \\
        \bottomrule
    \end{tabular}
    \caption{Model performance in micro F1 scores for the zero-shot (ZS) and cross-type transfer (CTT) test suites. ZS-1, ZS-5, and ZS-10 indicate 1, 5, and 10 event types for training respectively.
    We exclude TANL and DyGIE++ as they cannot transfer to unseen events.
    % \vspace{-4mm}
    % \tp{point for macro score}
    % \kw{add note for other models for not applicable.}
    }
    \label{tab:no-train-results}
    \vspace{-3mm}
\end{table}

\subsection{Analysis: Entity Breakdown}

\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lrrr}
        \toprule
         & \textbf{Entity} & \textbf{Non-entity} & \textbf{$\Delta$} \\
        \midrule
        DEGREE & 64.51 & 53.14 & 11.37 \\
        TANL & 68.16 & 59.1 & 9.06 \\
        BERT\_QA & 53.74 & 39.85 & 13.89 \\
        \bottomrule
    \end{tabular}
    \caption{Breakdown of micro F1 scores into entity and non-entity arguments for various EAE models trained on $1200$ samples. $\Delta$ is the difference.}
    \label{tab:entity-analysis}
    \vspace{-3mm}
\end{table}

In \dataName, we introduced non-entity arguments for the first time.
Non-entity arguments are more challenging to predict as they are more abstract and have longer spans.
To study how models perform on non-entity arguments, we break down the micro F1 performance of the models trained on $1200$ samples into entity and non-entity F1 scores, as shown in Table~\ref{tab:entity-analysis}.
We note that all models consistently perform better on entity arguments by a significant margin of $9$-$14$ F1 points.
Thus, more efforts need to be put in model designs to handle non-entity arguments better.

\subsection{Discussion}

\tp{Do we need this section as it's kind of a repetition of many takeaways in the results. What if we highlight the takeaways in bold}
% We conduct additional experiments to study the impact of reduced diversity and significance of diversity in \dataName{}, and report the results in Appendix~\ref{sec:pre-training} and ~\ref{sec:case-study-diversity}.
Overall, our generalizability experiments reveal many insights.
First, we observe the superior generalizability of \modelName{} owing to its natural language prompts.
Second, macro score evaluation reveals how models like TANL and DyGIE++ can be biased toward high-data events and exhibit poor generalization.
Finally, we note the advancement of generation-based models for better generalization.
% Overall, we observe better performance of generation-based models, like TANL and \modelName{} compared to classification-based models, like OneIE and DyGIE++ across all test suites.

% We show the model performance for \modelName and QAEE in the zero-shot test suite in Figure~\ref{fig:zero-shot-benchmarking}.
% Similar to the limited data setting, \modelName outperforms the other models and establishes its better generalizability.
% We further observe performance gains for all models as we increase the number of events in the training data (while keeping the training data size constant).
% On the other hand, these gains reduce as the number of training events increases.
% Thus, we conclude that event diversity helps improve zero-shot performance but provides marginally reducing gains.
% \tp{plot for zero-shot and numbers in table for cross-type transfer}

% We present the results for the cross-type transfer test-suite in Table~\ref{tab:ctt-results}.
%  (Table~\ref{tab:no-train-results}).
% The training data for this test suite comprises of all data for 9 events from the Scenario abstraction type (refer to Appendix~\ref{sec:event-organization}).
% Despite having a good amount of event diversity, we observe that the model performance is poorer for this test suite than the zero-shot test suite with similar number of events (ZS-5 and ZS-10).
% This highlights the additional challenge of transferring across different event types introduced by this test suite.

% We present the results for the cross-type transfer test-suite in Table~\ref{tab:ctt-results}.
% We observe that the \modelName shows great transfer capabilities as it outperforms the QAEE model by a significant margin.
% The training data for this test suite comprises of all data for 9 events from the Scenario abstraction type (refer to Appendix~\ref{sec:event-organization}).
% Despite having a good amount of event diversity, we observe that the model performance is poorer for this test suite than the zero-shot test suite with similar number of events.
% This highlights the additional challenge of transferring across different event types introduced by this test suite.

% We also observe that the pre-trained models outperform their respective models trained from scratch.
% The performance gains reduce as the number of training datapoints increase.
% This underlines how pre-training helps in better domain adaptation, and more especially in the low-resource setting.

% From the figures, we observe that when models are trained from scratch, \modelName outperforms other baseline models significantly on all sets of training event mentions.
% This trend also follows when the models are pre-trained on the ACE dataset.
% This highlights the generalizability and superior performance of \modelName (and generally generative approaches) over classification-based approaches.

% We also observe that the pre-trained models outperform their respective models trained from scratch.
% The performance gains reduce as the number of training datapoints increase.
% This underlines how pre-training helps in better domain adaptation, and more especially in the low-resource setting.

% \kw{Use three different figures to highlight individual aspects.}

% \paragraph{Uniform Sampling}
% In this setup, we uniformly sample equal number of event mentions per event and show the model performance results for micro-F1 in Figure~\ref{fig:uniform_sampling_micro_f1}.
% Similar to random sampling, we observe how \modelName outperforms other baseline models and also how pre-training helps improve model performance significantly.

% Overall, the best model F1 score with full training (the points on the extreme right) is still around 60 in Figure~\ref{fig:random_sampling_micro_f1}.
% This shows how \dataName is a challenging dataset and there is a large scope for overall improvement.

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lrrrr}
%         \toprule 
%         Model & LR & FS & ZS & CTT \\
%         \midrule
%         % OneIE & & \\
%         DyGIE++ & -4.56 & \textbf{1.02} & - & - \\
%         QAEE & -4.31 & -3.28 & -2.69 & -0.64 \\
%         \modelName & \textbf{-2.36} & -1.45 & \textbf{-0.62} & \textbf{-0.1}\\
%         \bottomrule
%     \end{tabular}
%     \caption{Average difference between the macro-F1 and micro-F1 scores for the models in the different benchmarking test suites. LR = low resource, FS = few-shot, ZS = zero-shot, and CTT = cross-type transfer.
%     % \tp{Add standard deviation as well if it's significant to show}
%     }
%     \label{tab:macro-f1-difference}
% \end{table}

% \subsection{Macro-F1 Analysis}

% Naturally, the trends of the model performance are similar across micro-F1 and macro-F1 scores and might not provide additional insights.
% Instead, we study the difference between the macro-F1 and the micro-F1 scores.
% A high difference (face value and not absolute terms) indicates a more uniform performance across all events and lesser bias towards events with higher data, which in turn, establishes better generalizability.
% We present the average difference between the scores for different models across different test suites in Table~\ref{tab:macro-f1-difference}.

% % In order to study the macro-F1 model performance, we show the average difference between the macro-F1 and micro-F1 scores of the different models in both the data setups in Table~\ref{tab:macro-f1-difference}.
% % A low macro-F1 score (or a highly negative difference) indicates a poor uniform performance across all event types which would be due to the bias of event types with higher datapoints.
% % We observe that the difference is negative most cases, which indicates that the micro-F1 is better than the macro-F1 scores.

% % \tp{This para will change according to results}
% Although DyGIE++ has a high positive difference in the few-shot setting, its absolute micro-F1 scores are super poor (as seen in Figure~\ref{fig:uniform_sampling_micro_f1}).
% Overall, we observe that \modelName has the highest difference across most benchmarking test suites.
% % We observe that in both sampling setups, the absolute difference is much lesser for \modelName compare to the other models.
% This emphasizes how \modelName generalizes uniformly across all event types.
% % We also observe a better difference in uniform sampling compared to random sampling setup.
% % This indicates how uniform sampling presents a good benchmarking test suite to evaluate the generalized model performance across all events.
% Across the different benchmarking suites, we observe that the difference is more in the no training data setting (ZS and CTT) compared to the limited training data setting (LR and FS).
% This disparity shows how training data can bias the models towards certain event types and hinder uniform model performance.
% \tp{Conclusion for previous observation. Overall, need a better table/conclusion for this part.}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/random-sampling-micro-f1.png}
%     \caption{Macro-F1 score distribution of the best trained models.}
%     \label{fig:macro-f1-distribution}
% \end{figure}

% \tp{We might add another paragraph to discuss the distribution of F1 scores between the models.}

% \subsection{Zero-shot Benchmarking}

% We show the main results for zero-shot benchmarking in Figure~\ref{fig:zero-shot-benchmarking}.
% Note that we used a fixed amount of training data while varying the number of training events.
% First, we observe that the \modelName outperforms the QAEE baseline significantly and shows good generalization even in the zero-shot setting.
% Secondly, we observe that the model performance difference doesn't vary significantly as we increase the number of events in the training data.
% This indicates that for the same amount of training data, increasing event diversity doesn't improve the performance much.
% \tp{Comment about model performance and pre-training}
% \ih{Need to add a bunch of other baselines for zero-shot claim}

% \tp{Paragraph and comments about how diversity of many event types affects model performance.}

% \subsection{Ablation Study of \modelName with \degree}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lr}
%         \toprule
%         & Micro-F1 \\
%         \midrule
%         DEGREE & 57.46 \\
%         \midrule
%         \quad w/ no event description & 57.32 \\
%         \quad w/ event type mention & 57.45 \\
%         \midrule
%         \quad w/ default mapping & 54.18 \\
%         \quad w/ argument mapping & 56.04 \\
%         \midrule
%         \quad w/ event-agnostic template & 59.04 \\
%         \midrule
%         \modelName & 56.62 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Ablation results for various automation heuristics experimented for automating the \degree model on the \ablationDataName dataset.}
%     \label{tab:automation-ablation}
% \end{table}

% As discussed in Section~\ref{sec:dam}, we introduce simple heuristics to automate the various manual components in prompt generation in the \degree model.
% % In order to evaluate the impact of these heuristics, we ablate each of these heuristics individually and compare them with model performance using the \degree model.
% Here, we provide an ablation study for each of these heuristics to evaluate their individual impact on the model performance.
% % We need to manually write descriptive prompts for each event type for the original \degree model.
% Since \degree requires manual annoation for each event type, we sample a small dataset \ablationDataName comprising of 10 event types from the original 
% We introduce a smaller dataset \ablationDataName comprising of 10 event types from the original FrameNet dataset for this ablation.
% We show these ablation results on the \ablationDataName dataset in Table~\ref{tab:automation-ablation}.

% First, we observe that automating event type description using no description or event type mention (second and third rows) yields very little performance difference.
% The major performance drop happens when automating argument role mapping and the corresponding results are shown in the fourth and fifth rows respectively.
% Surprisingly, we observe that replacing the original template with an event-agnostic template leads to an improvement in the performance.
% Overall, when we combine all these individual heuristics to get the \modelName model, we observe less than 1 point of F1 score dip.
% Thus, we show that \modelName scales up \degree while providing nearly similar performance.
% % \tp{Paragraph describing not much performance dip. Also write about ACE pre-training and comparable results there as well.}

% \subsection{Pre-training experiments}

% \tp{ACE v/s ERE v/s ACE-ERE}
